A search for hidden white dwarfs in the ROSAT EUV survey

The ROSAT WFC survey has provided us with evidence for the existence of a previously unidentified sample of hot white dwarfs (WD) in non-interacting binary systems, through the detection of EUV and soft X-ray emission. These stars are hidden at optical wavelengths due to their close proximity to much more luminous main sequence (MS) companions (spectral type K or earlier). However, for companions of spectral type A5 or later the white dwarfs are easily visible at far-UV wavelengths, and can be identified in spectra taken by IUE. Eleven white dwarf binary systems have previously been found in this way from ROSAT, EUVE and IUE observations (e.g. Barstow et al. 1994). In this paper we report the discovery of three more such systems through our programmes in recent episodes of IUE. The new binaries are HD2133, RE J0357+283 (whose existence was predicted by Jeffries, Burleigh and Robb 1996), and BD+27 1888. In addition, we have independently identified a fourth new WD+MS binary, RE J1027+322, which has also been reported in the literature by Genova et al. (1995), bringing the total number of such systems discovered as a result of the EUV surveys to fifteen. We also discuss here six stars which were observed as part of the programme, but where no white dwarf companion was found. Four of these are coronally active. Finally, we present an analysis of the WD+K0IV binary HD18131 (Vennes et al. 1995), which includes the ROSAT PSPC X-ray data.

==> tables.tex <==
\outer\def\section#1\par{\vskip0pt plus.3\vsize\penalty-25
  \vskip0pt plus-.3\vsize\bigskip\vskip\parskip
  \message{#1}\leftline{\bf#1}\nobreak\smallskip\noindent}
\outer\def\subsection#1\par{\vskip0pt plus.3\vsize\penalty-1
  \vskip0pt plus-.3\vsize\medskip\vskip\parskip
  \message{#1}\leftline{\bf#1}\nobreak\smallskip\noindent}\relax

\hoffset=-10mm\voffset=-13mm\hsize=180mm\nopagenumbers
\baselineskip=5.0mm\parindent=8mm\smallskipamount=8pt
\vsize=270mm

\settabs 7 \columns
\+ Table 1. ROSAT WFC/PSPC and EUVE count rates (1000s$^{-1}$) \cr
\vskip 0.5mm \hrule \vskip 0.5mm \hrule \vskip 0.5mm
\+ & WFC & & PSPC & & EUVE & \cr
\+ Name & S1 & S2 & (0.1-0.4keV) & (0.4-2.4keV) & 100\AA & 200\AA \cr
\vskip 0.5mm \hrule \vskip 0.5mm
\+ WD Binaries & & & & & & \cr
\+ HD2133 & 14$\pm$5 & 32$\pm$9 & 46$\pm$11 & no det. & no det. & no det. \cr
\+ HD18131 & 65$\pm$13 & 127$\pm$21 & 262$\pm$36 & 52$\pm$16 & 137$\pm$14
& 44$\pm$12 \cr
\+ RE J0357$+$283 & 46$\pm$9 & 55$\pm$10 & 210$\pm$29 & no det. & 54$\pm$11
 & no det. \cr
\+ BD$+$27$^\circ$1888 & 33$\pm$5 & 19$\pm$7 & 212$\pm$24 & no det. & 
46$\pm$10 & no det. \cr
\+ RE J1027+323 & 15$\pm$4 & 23$\pm$7 & 52$\pm$17 & no det. & 40$^*$ & no det. \cr
\+ Non-WD Systems & & & & & & \cr
\+ 2RE J0014$+$69$^{1}$ & no det. & 36$\pm$10 & no det. & no det. & no det. & no det. \cr
\+ CD$-$44 1025 & 25$\pm$6 & 27$\pm$6 & 693$\pm$47 & 575$\pm$41 & 36$\pm$7 
& no det. \cr
\+ HR1249 & 34$\pm$6 & 41$\pm$7 & 785$\pm$50 & 739$\pm$48 & 50$\pm$12 & no det. \cr
\+ HR2468 & 34$\pm$3 & 32$\pm$4 & 1389$\pm$38 & 919$\pm$31 & 47$\pm$4 &
9$\pm$4 \cr
\+ BD$-$00$^\circ$1462 & 13$\pm$3 & 26$^{\dag}$ & 196$\pm$28 & 134$\pm$22 &
no det. & no det. \cr
\+ RE J1809$+$29$^{2}$ & 26$\pm$4 & 51$\pm$13 & 307$\pm$21 & 197$\pm$17 & 25$\pm$7 &
no det. \cr
\vskip 0.5mm \hrule \vskip 0.5mm
\vskip 0.5mm \hrule \vskip 0.5mm
\+ * No error given in Bowyer et al. (1996), $^{\dag}$ upper limit \cr
\+ 1] AG$+$68 14 was observed as a possible counterpart to this source \cr 
\+ 2] HD166435 was observed as a possible counterpart to this source \cr

\vskip 10mm
\settabs 7 \columns
\+ Table 2. Log of IUE observations \cr
\vskip 0.5mm \hrule \vskip 0.5mm \hrule \vskip 0.5mm
\+ Name & IUE SWP No. & LWP No. & Date & Exposure (s) & Observer & notes \cr
\vskip 0.5mm \hrule \vskip 0.5mm
\+ WD Binaries & & & & & \cr
\+ HD2133 & 55659 & & 1995/234  & 1800 & Burleigh & \cr
\+ &  56231 & & 1995/329  & 2700 & SO & newsips \cr
\+ & & 31757 & 1995/329 & 600 & SO & newsips \cr
\+ HD18131 & 52151 & & 1994/266 & 5500 & Vennes & mildly saturated\cr
\+ & 52158 & & 1994/267 & 2000 & Byrne & \cr
\+ RE J0357$+$283 & 55660 & & 1995/234 & 3780 & Burleigh & \cr
\+ & & 26441 & 1993/265 & 1500 & Jeffries & \cr
\+ BD$+27$$^\circ1888$ & 49779 & & 1994/006 & 4000 & Burleigh & 2$\times$
over-exposed \cr
\+              & 49780 & & 1994/006 & 1200 & Burleigh & \cr
\+ & 56261 & & 1995/336 & 1200 & SO & newsips\cr
\+ & & 31785 & 1995/336 & 300 & SO & newsips\cr
\+RE J1027$+$322 & 49778 & & 1994/006 & 1200 & Burleigh &  \cr
\+              & 49793 & & 1994/008 & 11100 & Burleigh & \cr
\+              & 54501 & & 1995/115 & 7500 & Burleigh & newsips\cr
\+ Non-WD Systems & & & & & \cr
\+ AG$+$68 14 & 52807 & & 1994/319 & 1800 & Burleigh & \cr
\+ CD$-$44 1025 & 56046 & & 1995/274 &  900 & SO & newsips \cr
\+ & 56047 & & 1995/274 & 900 & SO & newsips \cr
\+ & & 31570 & 1995/274 & 35 & SO & newsips \cr
\+ HR1249 & 49792 & & 1994/008 & 2400 & Burleigh & \cr
\+ HR2468 & 52802 & & 1994/318 & 1800 & Burleigh & \cr
\+ BD$-$00$^\circ$1462 & 8200 & & 1980/069 & 3000 & Oranje  & \cr
\+ & 52801 & & 1994/318 & 1800 & Burleigh & \cr
\+ HD166435 & 55658 & & 1995/264 & 3600 & Burleigh & \cr
\vskip 0.5mm \hrule \vskip 0.5mm
\vskip 0.5mm \hrule \vskip 0.5mm
\+ SO$=$Service Observation \cr

\vskip 30mm
\settabs 6 \columns
\+ Table 3. Physical parameters of the companion stars in the binaries\cr
\vskip 0.5mm \hrule \vskip 0.5mm \hrule \vskip 0.5mm
\+ RE No. & Cat. Name & Spectral type &  V magnitude & d est. (pc) &
references \cr
\vskip 0.5mm \hrule \vskip 0.5mm
\+RE J0024$-$741 & HD2133 & F8V & 9.7 & 146 & \cr
\+RE J0254$-$053 & HD18131 & K0IV & 7.32 & 67 & 1 \cr
\+RE J0357$+$283 &        & K2V & 11.7 & $>$107 & 2\cr
\+RE J1024$+$262 & BD$+27$$^\circ1888$ & A8V-F2V & 9.1 & 185$-$218 & \cr
\+RE J1027$+$322 &        & G2($\pm$2)V & 13.0 & 380$-$550 & 3 \cr
\vskip 0.5mm \hrule \vskip 0.5mm 
\vskip 0.5mm \hrule \vskip 0.5mm
\+ Refs. 1] Vennes et al. (1995) 2] Jeffries, Burleigh \& Robb (1996)  
3]Genova et al. (1995) \cr

\vskip 10mm
\settabs 5 \columns
\+ Table 4. Physical parameters of the stars observed where no white
dwarf was detected \cr
\vskip 0.5mm \hrule \vskip 0.5mm \hrule \vskip 0.5mm
\+  RE No. & Cat. Name & Spectral type &  V magnitude & references \cr
\vskip 0.5mm \hrule \vskip 0.5mm
\+ 2RE J0014$+$691 & AG$+$68 14 & F8 & 10.3 & simbad \cr
\+ RE J0312$-$442 & CD$-$44 1025 & F3V$+$A8V & 5.93 & simbad \cr
\+ RE J0402$-$001 & HR1249 & F6V & 5.38 & simbad \cr
\+ RE J0637$-$613 & HR2468 & G1.5V & 6.18 & simbad \cr
\+ RE J0650$-$003 & BD$-$00$^\circ$1462 & F2V & 5.77 & simbad \cr
\+ RE J1809$+$295 & HD166435 & G0 & 6.84 & simbad \cr
\vskip 0.5mm \hrule \vskip 0.5mm
\vskip 0.5mm \hrule \vskip 0.5mm

\vskip 200mm
\settabs 8\columns
\+ Table 5. Temperatures and gravities for the white dwarfs from
homogeneous model fits\cr
\vskip 0.5mm \hrule \vskip 0.5mm \hrule \vskip 0.5mm
\+ Binary & log g &  Temp & 90\% error & Mass & Radius & d $\sb {wd}$ & Estimated V \cr
\+     &  & K & K & M$_\odot$ & R$_\odot$ & (pc) & \cr
\vskip 0.5mm \hrule \vskip 0.5mm
\+ HD2133 & 7.0 & 24,490 & 24,160-24,870 & 0.37 & 0.032 & 234 & 15.4\cr
\+ & 7.5 & 26,420 & 26,100-26,810 & 0.42 & 0.019 & 165 & 15.6 \cr
\+ & 7.75 & 26,780 & 26,510-27,270 & 0.52 & 0.016 & 139 & 15.6 \cr
\+ & 8.0 & 28,260 & 27,910-28,630 & 0.65 & 0.013 & 132 &  15.7 \cr
\+ & 8.25 & 28,700 & 28,350-29,050 & 0.79 & 0.011 & 112 & 15.7 \cr
\+ & 8.5 & 29,900 & 29,560-30,400 & 0.95 & 0.009 & 100 &  15.8 \cr
\+ & 9.0 & 31,650 & 31,240-32,260 & 1.20 & 0.006 & 68 &  15.9 \cr
\+ & & & & & & & & & &  \cr
\+ HD18131 & 7.0 & 26,440 & 26,170-26,740 & 0.37 & 0.032 & 126 & 13.9 \cr
\+ & 7.5 & 29,290 & 28,650-29,640 & 0.43 & 0.019 & 93 & 14.1 \cr
\+ & 8.0 & 31,130 & 30,750-31,540 & 0.65 & 0.013 & 72 & 14.2 \cr
\+ & 8.5 & 32,980 & 32,530-33,470 & 0.95 & 0.009 & 53 & 14.2 \cr
\+ & 9.0 & 35,050 & 34,500-35,640 & 1.20 & 0.005 & 36 & 14.3 \cr
\+ & & & & & & & & & &  \cr
\+ RE J0357+28 & 7.0 & 27,330 & 27,050-27,640 & 0.37 & 0.032 & 185 & 14.6 \cr
\+ & 7.5 & 29,460 & 29,130-29,820 & 0.43 & 0.019 & 130 & 14.8 \cr
\+ & 7.9 & 30,960 & 30,620-31,410 & 0.60 & 0.014 & 105 & 14.9 \cr
\+ & 8.0 & 31,340 & 30,940-31,760 & 0.65 & 0.013 & 100 &  14.9 \cr
\+ & 8.5 & 33,430 & 32,950-33,950 & 0.95 & 0.009 & 75 &  14.9 \cr
\+ & 9.0 & 35,840 & 35,240-36,540 & 1.20 & 0.005 & 51 &  15.0 \cr
\+ & & & & & & & & & &   \cr
\+ BD$+27$$^\circ1888$ & 7.0 & 33,180 & 32,340-34,380 & 
0.38 & 0.032 & 242 & 14.8 \cr
\+ & 7.25 & 34,130 & 33,330-35,780 & 0.39 & 0.025 & 193 & 14.8 \cr
\+ & 7.5 & 35,370 & 34,530-37,300 & 0.45 & 0.020 & 162 & 14.9 \cr
\+ & 8.0 & 38,420 & 37,330-40,870 & 0.67 & 0.014 & 120 & 14.9  \cr
\+ & 8.5 & 42,470 & 41,050-45,690 & 0.96 & 0.009 & 89 & 15.0 \cr
\+ & 9.0 & 47,640 & 45,800-51,790 & 1.21 & 0.005 & 61 & 15.1 \cr
\+ & & & & & & & & & & \cr
\+ RE J1027+32 & 7.0 & 30,560 & 29,560-32,600 & 
0.37 & 0.032 & 589 & 16.9 \cr
\+ & 7.25 & 32,265 & 30,760-33,500 & 0.39 & 0.025 & 487 & 16.9 \cr
\+ & 7.5 & 32,440 & 31,570-34,450 & 0.44 & 0.020 & 388 & 16.9 \cr
\+ & 8.0 & 34,000 & 33,400-36,460 & 0.66 & 0.013 & 288 & 17.0 \cr
\+ & 8.5 & 37,020 & 35,620-38,650 & 0.96 & 0.009 & 216 & 17.1 \cr
\+ & 9.0 & 39,240 & 37,910-41,380 & 1.20 & 0.005 & 144 & 17.2 \cr
\vskip 0.5mm \hrule \vskip 0.5mm
\vskip 0.5mm \hrule \vskip 0.5mm


\vskip 120mm
\settabs 7 \columns
\+ Table 6. He/H ratios and column densities from homogeneous models \cr
\vskip 0.5mm \hrule \vskip 0.5mm \hrule \vskip 0.5mm
\+ Name & log g & T & He/H & HI column & $\chi_r$$^2$ & Comment \cr
\vskip 0.5mm \hrule \vskip 0.5mm
\+ HD2133 & 7.0 & 24,490 & - & - & 19.2 & No Fit \cr  
\+ & 7.5 & 26,420 & 1$\times$10$^{-8}$ & 0.0 & 2.71 & \cr
\+ & 7.75 & 26,780 & 1.35$\times$10$^{-7}$ & 0.0 & 0.79 & \cr
\+  & 8.0 & 28,260 & 1.29$\times$10$^{-5}$ & 1.58$\times$10$^{18}$ & 0.54  & \cr
\+ & 8.25 & 28,700 & 3.00$\times$10$^{-5}$ & 0.0 & 0.63 & \cr
\+ & 8.5 & 29,900 & 5.89$\times$10$^{-5}$ & 0.0 & 1.56 & \cr
\+ & 9.0 & 31,460 & - & - & 8.44 & No Fit \cr
\+ & & & & & & \cr
\+ HD18131 & 7.0 & 26,440 & - & - & 17.0 & No Fit \cr
\+ & 7.5 & 29,290 & 1$\times$10$^{-8}$ & 1.17$\times$10$^{19}$ & 1.61 & \cr
\+ & 8.0 & 31,130 & 3.63$\times$10$^{-5}$ & 7.20$\times$10$^{18}$ & 1.17 & \cr
\+ & 8.5 & 32,980 & 2.29$\times$10$^{-4}$ & 0.0 & 3.64 & \cr
\+ & 9.0 & 35,050 & 4.90$\times$10$^{-3}$ & 0.0 & 2.31 & \cr
\+ & & & & & & \cr
\+ RE J0357$+$283 & 7.0 & 27,330 & - & - & 22.9 & No Fit \cr
\+ & 7.5 & 29,460 & - & - & 11.4 & No Fit \cr
\+ & 7.9 & 30,960 & 6.67$\times$10$^{-5}$ & 2.10$\times$10$^{19}$ & 4.27 & \cr
\+ & 8.0 & 31,340 & 6.90$\times$10$^{-5}$ & 2.27$\times$10$^{19}$ & 3.16 & \cr
\+ & 8.5 & 33,430 & 7.33$\times$10$^{-5}$ & 1.92$\times$10$^{19}$ & 2.08 & \cr
\+ & 9.0 & 35,840 & 6.91$\times$10$^{-5}$ & 1.02$\times$10$^{19}$ & 2.42 & \cr
\+ & & & & & & \cr
\+BD$+$27$^\circ$1888 & 7.0 & 33,180 & - & - & 17.5 & No Fit \cr
\+ & 7.25 & 34,130 & 9.8$\times$10$^{-7}$ & 3.31$\times$10$^{19}$ & 3.28 & \cr
\+ & 7.5 & 35,370 & 1$\times$10$^{-8}$ & 4.79$\times$10$^{19}$ & 3.87 & \cr
\+ & 8.0 & 38,420 & 1$\times$10$^{-8}$  & 7.25$\times$10$^{19}$ & 6.27 &  \cr 
\+ & 8.5 & 42,470 & - & - & 22.7 & No Fit \cr
\+ & 9.0 & 47,640 & - & - & 31.0 & No Fit \cr
\+ & & & & & & \cr
\+ RE J1027$+$323 & 7.0 & 30,560 & 1.0$\times$10$^{-8}$ & 2.86$\times$10$^{18}$ & 5.85 & \cr
\+  & 7.25 & 32,265 & 9.55$\times$10$^{-7}$ & 8.24$\times$10$^{18}$ & 3.31 & \cr
\+ & 7.5 & 32,440 & 4.78$\times$10$^{-7}$ & 1.05$\times$10$^{19}$ & 2.38 & \cr
\+ & 8.0 & 34,000 & 1.0$\times$10$^{-8}$ & 1.66$\times$10$^{19}$ & 1.25 & \cr
\+ & 8.5 & 37,020 & 2.51$\times$10$^{-4}$ & 0.0 & 2.04 & \cr
\+ & 9.0 & 39,240 & 5.75$\times$10$^{-4}$ & 0.0 & 3.24 & \cr
\+ & & & & & & \cr
\vskip 0.5mm \hrule \vskip 0.5mm
\vskip 0.5mm \hrule \vskip 0.5mm

\vskip 120mm
\settabs 5 \columns
\+ Table 7. BD$+$27$^\circ$1888: Comparison between the temperatures
derived 
from fitting SWP49780 and SWP56261 (NEWSIPS) \cr
\vskip 0.5mm \hrule \vskip 0.5mm \hrule \vskip 0.5mm
\+ & SWP49780 & & SWP56261 &  \cr
\+ log g & Temp & 90\% Range & Temp & 90\% Range \cr
\vskip 0.5mm \hrule \vskip 0.5mm 
\+ 7.0 & 27,620 & 26,760-29,140 & 33,180 & 32,340-34,380 \cr
\+ 7.5 & 30,400 & 29,220-31,470 & 35,370 & 34,530-37,300 \cr
\+ 8.0 & 31,980 & 31,000-33,480 & 38,420 & 37,330-40,870 \cr
\+ 8.5 & 34,390 & 33,080-35,865 & 42,470 & 41,050-45,690 \cr
\+ 9.0 & 37,180 & 35,615-38,740 & 47,640 & 45,800-51,790 \cr 
\vskip 0.5mm \hrule \vskip 0.5mm
\vskip 0.5mm \hrule \vskip 0.5mm


\vskip 10mm
\settabs 5 \columns
\+ Table 8. Line fluxes for the active stars observed with IUE \cr
\vskip 0.5mm \hrule \vskip 0.5mm \hrule \vskip 0.5mm
\+ Name & CII$^*$ & SiIV$^*$ & CIV$^*$ & HeII$^*$ \cr
\+ 	& 1335\AA & 1397\AA & 1549\AA & 1640\AA   \cr
\vskip 0.5mm \hrule \vskip 0.5mm
\+ HD39587$^+$ & 4.02$\pm$0.12 & 4.01$\pm$ 0.14 & 5.15$\pm$0.14 & 2.50$\pm$0.11
 \cr
\+ HD126660$^+$ & 6.21$\pm$0.5 & 4.74$\pm$0.34 & 10.4$\pm$0.62 &
2.91$\pm$0.5 \cr
\+ CD$-$44 1025 & - & - & 4.40$\pm$0.67 & 1.35$\pm$0.40 \cr
\+ HR1249 & 1.83$\pm$0.24 & 3.67$\pm$0.43 & 4.11$\pm$0.35 & 0.75$\pm$0.21 \cr
\+ HR2468 & 1.26$\pm$0.22 & - & 2.89$\pm$0.4 & 1.26$\pm$0.29 \cr
\+ BD$-$00$^\circ$1462 & - & - & 1.82$\pm$0.34$^{\dag}$ & - \cr
\vskip 0.5mm \hrule \vskip 0.5mm
\vskip 0.5mm \hrule \vskip 0.5mm
\+ $^*$ $\times$10$^{-13}$ ergs/cm$^2$/sec, $^+$ comparison star (see
text), $^{\dag}$ possible detection \cr

\vskip 10mm
\settabs 6 \columns
\+ Table 9. EUV and X-ray luminosities for the active stars observed\cr
\vskip 0.5mm \hrule \vskip 0.5mm \hrule \vskip 0.5mm
\+ Name & d(pc) & L$_{EUV}$ & L$_{EUV}$/L$_{bol}$ & L$_x$ &
L$_x$/L$_{bol}$ \cr
\+ & & $\times$10$^{29}$ ergs & $\times$10$^{-5}$ & $\times$10$^{29}$ ergs & 
$\times$10$^{-5}$ \cr
\vskip 0.5mm \hrule \vskip 0.5mm
\+ HD39587$^+$ & 11 & 0.8 & 1.2 & 1.9  & 3.0 \cr
\+ HD126660$^+$ & 12 & 0.9 & 0.8 & 2.9 & 2.8 \cr
\+ CD$-$44 1025(F3V) & 37 & 6.6  & 3.8 & 16.7 & 9.6 \cr
\+ CD$-$44 1025(A8V) & 51 & 12.6 & 3.5 & 31.7 & 8.8 \cr
\+ HR1249 & 23 & 3.9 & 3.5 & 7.9 & 7.1 \cr
\+ HR2468 & 23 & 3.0 & 5.5 & 10.9 & 19.7 \cr
\+ BD$-$00$^\circ$1462 & 36 & 6.0$^{\dag}$ & 3.1$^{\dag}$ & 3.8 & 2.0 \cr
\vskip 0.5mm \hrule \vskip 0.5mm
\vskip 0.5mm \hrule \vskip 0.5mm
\+ $^+$ comparison star (see text), $\dag$ upper limit \cr

\end

